Proteus: Preserving Model Confidentiality during Graph Optimizations

Deep learning (DL) models have revolutionized numerous domains, yet optimizing them for computational efficiency remains a challenging endeavor. Development of new DL models typically involves two parties: the model developers and performance optimizers. The collaboration between the parties often necessitates the model developers exposing the model architecture and computational graph to the optimizers. However, this exposure is undesirable since the model architecture is an important intellectual property, and its innovations require significant investments and expertise. During the exchange, the model is also vulnerable to adversarial attacks via model stealing. This paper presents Proteus, a novel mechanism that enables model optimization by an independent party while preserving the confidentiality of the model architecture. Proteus obfuscates the protected model by partitioning its computational graph into subgraphs and concealing each subgraph within a large pool of generated realistic subgraphs that cannot be easily distinguished from the original. We evaluate Proteus on a range of DNNs, demonstrating its efficacy in preserving confidentiality without compromising performance optimization opportunities. Proteus effectively hides the model as one alternative among up to $10^{32}$ possible model architectures, and is resilient against attacks with a learning-based adversary. We also demonstrate that heuristic based and manual approaches are ineffective in identifying the protected model. To our knowledge, Proteus is the first work that tackles the challenge of model confidentiality during performance optimization. Proteus will be open-sourced for direct use and experimentation, with easy integration with compilers such as ONNXRuntime.

==> sections/6_related_works.tex <==
\section{Related Work}

To our knowledge, our work is the first to (i) examine and analyze confidentiality challenges when applying graph-level optimizations in DL models, and (ii) propose a novel effective obfuscation mechanism to preserve confidentiality in any arbitrary DL model. We briefly discuss related works.

\textbf{Deep Learning Compilers.} Deep learning (DL) compilers~\cite{tvm,taso,ding2023hidet,sabne2020xla} provide graph-level and operator-level optimizations in the computational graphs to improve system performance in DL models. To do so, either the compiler itself is provided to the model-owner, or the end-to-end optimization process is completely performed by the optimizer party.
In contrast, \codename preserves the confidentiality of DL models, without (i) limiting the compilation-level optimizations that can be performed in DL models and (ii) requiring the optimizer party to provide the compiler (or the private compilation-level optimizations) to the model owner. Thus, \codename is orthogonal to DL compilers: \codename preserves the confidentiality of any arbitrary DL model, while DL compilers perform various graph-level optimizations to improve the performance of arbitrary DL models.

\textbf{Differential Privacy.}
Differential Privacy (DP)~\cite{dwork2006differential,dwork2014algorithmic} provides private data analysis, i.e., extracting useful statistics and information from a dataset, while protecting the identity and privacy of individuals in the dataset. 
However, DP-based solutions cannot fundamentally solve the confidentiality challenge in optimizing DL models: in the DL model optimization problem, the protected graph (DL model) needs to remain unchanged. Applying probabilistic perturbation DP methods would result in modifying the computations (calculations) performed by the protected DL model, thus violating the functional correctness of the DL model.

